Parallel Integer Polynomial Multiplication

We propose a new algorithm for multiplying dense polynomials with integer coefficients in a parallel fashion, targeting multi-core processor architectures. Complexity estimates and experimental comparisons demonstrate the advantages of this new approach.

==> cmmxx-implementation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:cmmxxmultiplication-implementation}

\ifthesis
We have implemented the proposed algorithm using {\sf CilkPlus} targeting multi-cores. 
The code for Convert-in and Convert-out steps can be found in Appendix~\ref{appendix:convert}.
\fi


==> cmmxx-standard-algorithms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Parallelization of Standard Multiplication Algorithms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{sec:multiplication-standard-algorithms}

